Skew-Oblivious Data Routing for Data-Intensive Applications on FPGAs with HLS

FPGAs have become emerging computing infrastructures for accelerating applications in datacenters. Meanwhile, high-level synthesis (HLS) tools have been proposed to ease the programming of FPGAs. Even with HLS, irregular data-intensive applications require explicit optimizations, among which multiple processing elements (PEs) with each owning a private BRAM-based buffer are usually adopted to process multiple data per cycle. Data routing, which dynamically dispatches multiple data to designated PEs, avoids data replication in buffers compared to statically assigning data to PEs, hence saving BRAM usage. However, the workload imbalance among PEs vastly diminishes performance when processing skew datasets. In this paper, we propose a skew-oblivious data routing architecture that allocates secondary PEs and schedules them to share the workload of the overloaded PEs at run-time. In addition, we integrate the proposed architecture into a framework called Ditto to minimize the development efforts for applications that require skew handling. We evaluate Ditto on five commonly used applications: histogram building, data partitioning, pagerank, heavy hitter detection and hyperloglog. The results demonstrate that the generated implementations are robust to skew datasets and outperform the stateof-the-art designs in both throughput and BRAM usage efficiency.

==> backup/background.tex <==
\section{background}\label{sec:background}

\subsection{HLS for FPGAs}\label{sec:hls}
Traditionally, HDLs like VHDL and Verilog are used as the programming language for FPGAs. However, coding with HDLs is time-consuming and tedious and requires an in-depth understanding of underlying hardware to maximize the performance. 
To alleviate this programming gap and boost the adoption of FPGA acceleration, FPGA vendors and research communities have been actively working on developing HLS tools which can translate a design description in high level languages (HLL) like C/C++ to a synthesizable implementation for the selected hardware. HLS tools enable data scientists to gain performance and energy benefits of FPGAs without investing lot of time and effort into learning hardware concepts. 
Intel has developed and released an extension to OpenCL which was initially developed for CPUs and GPUs to support their FPGAs~\cite{SDKdocument2018}, and Xilinx has SDAccel~\cite{SDAccel} tool chain which supports C/C++/System C and has recently added support for OpenCL as well. Andrew et al. are developing LegUp~\cite{legup}. 


\subsection{Execution Models of OpenCL}

==> backup/motivaton_bk.tex <==
\section{Motivation}\label{sec:motivation}
In this section, we illustrate the motivation of the skew-oblivious data routing with an example, data partitioning (DP) which is an important operator for in-memory analytical database engines. 

\subsection{Data Routing based DP with HLS}
Listing~\ref{list:datapartitioning} shows the algorithm of DP with data buffering enabled. The tuples are sequentially read from global memory, and indices of destination partitions are calculated through a hash function. Specially, the tuple is temporally buffered in the corresponding buffer and written out to the partition only when the buffer is full. The buffer size is usually of the size of a cache line for high memory efficiency. 

\begin{lstlisting}[language=C++, caption=Code snippet of data partitioning.,label={list:datapartitioning}]
for(i = 0; i < num_tuples; i ++){ 
    tuple = relation[i];
    idx = hash(tuple.key);     
    buffer[idx][(count[idx] ++) % N] = tuple;     
    if(count[idx] == N) 
        write out buffer[idx] to partition[idx];
}
\end{lstlisting}

Figure~\ref{fig:datapartitioning_independentPE} shows the state-of-the-art RTL-based design of DP~\cite{kara2017fpga}. 
Multiple tuples are read per cycle and sliced to multiple PEs. Each PE maintains buffers for all partitions and gathers the tuples to corresponding buffers. 
Importantly, a coordinator handles the runtime data dependency to synchronize the write index of a full buffer from any PE. 
Unfortunately, the coordinator is implemented with fine-grained control logic with HDL, which is inapplicable for HLS~\cite{Li2017}. 
As an evidence, the state-of-the-art HLS-based DP~\cite{Wang2017} only achieves a half of the theoretical performance. 

Figure~\ref{fig:datapartitioning_datarouting} depicts the proposed DP with HLS-based data routing logic.
The core idea is that each PE processes its own tuples, and the tuples are routed to designated PEs. 
In this way, PEs independently write buffers to the global memory without coordination. 
More importantly, the fan-out it can process is up to $(M + 1) \times N$, which is $(M + 1)$ times of the architecture without data routing~\cite{kara2017fpga} ($(M + 1)$ is usually around 8 or 16). 
%In the end, it requires less passes of partitioning for big datasets. 
%However, there is no vendor-specific extensions for data routing~\cite{kapre2017applying} and HLS tools could not extract the parallelism of functions with run-time data dependency~\cite{Li2017}. In this paper, we will propose flexible and efficient data routing logic for HLS tools, which is inspired by Chen et al.~\cite{chen2019fly}. 

\begin{figure}[h]
    \centering
    %\hline
    \begin{subfigure}[t]{0.23\textwidth}
        \centering
        %\smallskip
        \includegraphics[width=1\linewidth]{Figures/hist_indepdentPE-crop.pdf}
        \caption{SOTA RTL-based design.} %{Light Unit}
        \label{fig:datapartitioning_independentPE}
    \end{subfigure}
    \smallskip
    \begin{subfigure}[t]{0.23\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{Figures/hist_datarouting-crop.pdf}
        \caption{Design with data routing.}
        \label{fig:datapartitioning_datarouting}
    \end{subfigure}
%\hline
    \caption{Architectures with M+1 PEs for data partitioning.}
    \label{fig:archs_datapartitioning}   
\end{figure}

\subsection{Workload Imbalance Problem of Data Routing}
We have implemented data routing based DP with 16 PEs for tuple with 8-byte data width on our hardware platform (shown in Section~\ref{sec:hardware}).
We then profile the implementation under the dataset with 256$\times$1024$\times$100 tuples following the Zipf distribution.
Based on the profiling results, we have the following two observations. 

\vspace{1mm}
\noindent\textit{Observation 1: Data skew downgrades the throughput significantly.}
Figure~\ref{fig:ThroughputwithzipfDP} shows that the throughput of DP is downgraded significantly with increasing the Zipf factor, $\alpha$ from 0 to 3. 
%Since each PE processes exclusive data, with skew datasets, some PEs have a lot of data to process while others not. 
%In the end, the performance will be constrained to the PE which has the most of data to process.
The bigger the Zipf factor is, the more severe the imbalance is.  
The performance of extreme skew dataset ($\alpha = 3$) is only of the one-sixteenth of the performance under the uniformly distributed dataset ($\alpha = 0$) since almost all the data go to the same PE.

\vspace{1mm}
\noindent\textit{Observation 2: The overloaded PEs are varying with datasets.}
Figure~\ref{fig:workloaddistributionDP} shows the workload distribution (number of tuples) among PEs on skew datasets. 
The present number is calculated by the workload under skew datasets ($\alpha$ from \numrange{1}{3}) divided by that of the uniformly distributed dataset ($\alpha = 0$), and the decimal place is capped to one. The red color indicates PEs are overloaded while the green color under-utilized, the deeper color the heavier. 
It is clear over-loaded PEs are varying depending on the datasets; hence, statically increasing the processing capacity of specific PEs could not improve the throughput of evolving datasets. 

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.22\textwidth}
        \centering
        \includegraphics[width=1\linewidth]{Figures/motivation_zipf_throughput-crop.pdf}
        \caption{Throughput of DP with varying Zipf factor.} %{Light Unit}
        \label{fig:ThroughputwithzipfDP}
    \end{subfigure}
    \smallskip
    \begin{subfigure}[t]{0.25\textwidth}
        \centering
        \includegraphics[width=1\textwidth]{Figures/heatmap-crop.pdf}
        \caption{Workload distribution among 16 PEs.}
        \label{fig:workloaddistributionDP}
    \end{subfigure}
%\hline
    \caption{Profiling results with DP on Zipf datasets.}
    \label{fig:archs_datapartitioning}   
\end{figure}

\vspace{1mm}
\noindent\textbf{Data routing with skew handling.}
A natural solution is the work stealing, where the under-utilized PEs steal the data from over-loaded PEs. 
However, data-intensive applications on FPGA are BRAM read/write ports bounded~\cite{cong2018automated} instead of computation bounded.
As a result, working stealing will not pay off since it needs to write back to the buffer of the over-loaded PEs. 
On the contrary, increasing the BRAM read/write ports for over-loaded PEs is the fundamental way to solve the problem.
%or increase the BRAM bank for PEs...

To achieve that, we pre-allocate secondary PEs which also own private buffers and dynamically schedule them to the over-loaded primary PEs to increase the throughput. 
Primary PEs could process the full range of the data while secondary PEs process the same data with specific primary PEs.
Hence, the number of allocated secondary PEs trades off the dataset processed on-chip and the data skew the architecture can handle. 
%Furthermore, as the datasets are evolving and overloaded PEs are varying, our adaptive skew-oblivious data routing architecture schedules the secondary PEs to over-loaded PEs according to the dataset at run-time without re-synthesize.

Regardless of the adaptive data routing logic to skew datasets, there are still many tuning knobs involving a lot of application to hardware transformations such as memory optimizations and efficient data flow for HLS-based designs~\cite{cong2018automated}.
In this paper, we further integrate the adaptive data routing with skew handling and many tuning optimizations into a framework, called \textit{HHLS}, to assist developers to deploy applications that take the advantages of HLS and data routing on FPGAs.  
%We hence propose the framework, HHLS. 






==> commented.tex <==
\subsection{Applications} 
We use six widely used applications in datacenters to evaluate the efficiency of our framework, which are  Histogram Building (HISTO), Data Partitioning (DP), PageRank (PR), Hyperloglog (HLL), Heavyhitter Detection (HD) and Hash Joins (HJ).
Two of them are used in-network processing. 

\vspace{1mm}
\noindent\textbf{Histogram Building (HISTO).} 
The histogram could approximately represent the distribution of numerical data.
It plays an important role in many applications. For example, it helps modern database systems to optimize the query plan and schedule the computing resources.
There are many variants of histograms. In this paper, we evaluate the equi-width histogram~\cite{istvan2014histograms} where the value range of the dataset is evenly divided into multiple buckets, and each buckets counts the number of occurrences of the values under current range.

\vspace{1mm}
\noindent\textbf{Data Partitioning (DP).} 
Data partitioning which separates the big dataset into multiple chunks has been a very important operator for modern database systems. 
For example, it is involved in partition hash join, or used for partitioning the big data into multiple machines when processing at scale. 
In this paper, we adopt the data partitioning with radix hash function, following work~\cite{Wang2017,kara2017fpga}. Note that other hash functions can be also applied without sacrificing performance since they are pipelined in FPGA. 

\vspace{1mm}
\noindent\textbf{PageRank (PR).} 
PageRank is an important graph processing algorithm invented by Google. 
It works on graph dataset which is composed by nodes and their connections. 
The basic idea behind PageRank is each vertex node propagates its weight to their neighbours (the nodes connected with it). In this way, it could identify the importance of each node. 

\vspace{1mm}
\noindent\textbf{Hyperloglog (HLL).} 
HLL has been a standard algorithm to estimate the cardinality of a multiset, nowadays. 
For example, Google uses HLL in BigQuery, a cloud-based distributed data processing system. 
HLL provides approximate estimation on cardinality.
Since it requires small memory consumption while guarantee the enough accuracy for final estimation, it is very suitable to process in network with all the data in on-chip RAMs of FPGAs.   

\vspace{1mm}
\noindent\textbf{Sketch-based Heavyhitter Detection (HD).} 
Heavy hitter detection is the basis for many network management and security applications. Sketch-based Heavyhitter Detection is used to detect heavy hitters in network.

\vspace{1mm}
\noindent\textbf{Hash Joins (HJ).} 
The hash join, which joins two relations into one with respect to the common attribute, is a key operator in databases, and constitutes a significant portion of the execution time of a query. 

The notation of all the parameters is shown in Table~\ref{table:notation}.
\begin{table}[ht]
\centering
\caption{Notation of the parameters in the architecture.}
\label{table:notation}
\begin{tabular}{l|l}
\hline
Parameter  & Description  \\
\hline 
$Freq$     & frequency of the implementation \\
$Trip$             & trip counter of a loop \\
$Unroll$         &  unroll factor of a loop \\ 

$T$     & estimated execution time \\
$T_{read}$  &  estimated memory read time \\   
$T_{write}$     &  estimated memory write time   \\
$T_{process}$   &  estimated process time of the circuit    \\ 
$L$             &   latency of a stage or worker \\

$N_{input}$    &   number of input data \\
$S_{input}$    &   size of input data \\
$N_{output}$    &   number of output data \\ 
$S_{output}$    &   size of output data \\

$R_{input}$    &   randomness ratio of input data  \\
$R_{output}$    &   randomness ratio of output data  \\ 

$B(R)_{read}$    &  read bandwidth given the randomness of input \\
$B(R)_{write}$    & write bandwidth the randomness of output\\
$II$    &  The initiation interval of a loop   \\
$N_{worker_N}$    &  number of $Worker_n$\\

\hline
\end{tabular}
\end{table}


\begin{figure}[]
    \centering
    \begin{subfigure}[b]{0.4\linewidth}
    \includegraphics[width=1\linewidth]{Figures/mapper-crop.pdf}
    \caption{The mapping process.} %{Light Unit}
    \label{fig:mappertableupdate}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.5\linewidth}
    \includegraphics[width=1\linewidth]{Figures/mapper_workflow-crop.pdf}
    \caption{The map table output.} %{Light Unit}
    \label{fig:mapperprocess}
    \end{subfigure}
    \caption{The map table update.} %{Light Unit}
\end{figure}

\noindent\textbf{HISTO}
According to opensourced code of work~\cite{jiang2020boyi}, PEs are independent and the results of PEs are merged on CPU side.
The benefits with our framework are two folders: firstly, \textit{the computation does not involve CPU}; secondly, our implementation has 4,096$\times$ more buckets than theirs, \textit{achieving a more fine-grained distribution.}

\noindent\textbf{DP}
The RTL-based work~\cite{kara2017fpga} relies on fine-grained control logic for coordination among PEs. With our framework, the coordination is resolved for HLS; hence the implementation could also fully utilize the memory bandwidth. More importantly, our design could handle 8$\times$ bigger fan-out compared to work~\cite{kara2017fpga}, \textit{which reduces the number of passes of partitioning for large datasets.} 

%Note that the work~\cite{kara2017fpga} uses different platforms which has less memory bandwidth but their platform has unique feature that randomness does not influence the bandwidth too much. Overall, both two works could claim the system bottleneck is on memory interface instead of the logic inside of FPGA, but our implementation utilizes the on-chip RAMs better hence a bigger fanout.

\noindent\textbf{PR}
Although the performance is comparable with work~\cite{chen2019fly} as both adopt data routing architecture, \textit{we shall show our design outperforms them under super skewed graph datasets in the next section.}

\noindent\textbf{HLL}
Compare with RTL based work~\cite{hyperloglog}, our implementation could accommodate 16$\times$ more buckets; hence, \textit{it achieves much higher accurate cardinality estimation which is essential for large datasets.}

\noindent\textbf{HHD}
The work~\cite{heavyhitter} only has one pipeline which cannot fully utilize the bandwidth. With our framework, the implementation has multiple pipeline such that \textit{it can process finer grained tuples and sustain the bandwidth}. In addition, with data routing, \textit{our design could output the detected heavy hitters immediately instead of waiting for all the tuple processed and merging the buckets}.

\begin{table}[ht]
\caption{Resource utilization and frequency.}
\label{table:Resource-utilization}
\resizebox{0.475\textwidth}{!}{%
\begin{tabular}{lllllll}
\toprule
\multicolumn{1}{l}{Application}   & Frequency & RAM  & Logic & DSP   \\ \midrule
\multicolumn{1}{l|}{HISTO} & 237 MHz    & 383 (14\%) & 100,319 (23\%) & 0 (0\%) \\
\multicolumn{1}{l|}{DP}    & 208 MHz    & 711 (26\%) & 258,449 (60\%) & 32 (2\%) \\
\multicolumn{1}{l|}{PR}    & 176 MHz    & 1,195 (44\%) & 192,560 (45\%) & 80 (5\%) \\
\multicolumn{1}{l|}{HLL}   & 252 MHz    & 885 (33\%) & 170,325 (40\%) & 403 (27\%) \\ 
\multicolumn{1}{l|}{HD}    & 191 MHz    & 638 (24\%) & 148,782 (35\%) & 128 (8\%)  \\ 
\bottomrule
\end{tabular}%
}
\end{table}

\begin{equation}\label{eq:imp_select}
  {N_{secPE}} = \sum_{i=1}^{N_{priPE}}ceil(\frac{profiled\_workload_{priPE\_{i}}}{uniform\_workload}) - N_{priPE}
\end{equation}
\begin{equation}\label{eq:imp_select}
  {total\_workload}= \sum_{i=1}^{M} {workload_{priPE\_{i}}}
\end{equation}

